ExplainGuard: A Zero Trust Framework for Post-Hoc Explanation Integrity Guarantees in Blackbox XAI Models

As machine learning (ML) models are increasingly deployed in high-stakes environments, explainable AI (XAI) methods like SHAP and LIME have become essential for regulatory compliance and trust. However, the current auditing paradigm relies on an implicit "chain of trust" where third-party auditors are assumed to be trusted. Recent research demonstrates that this assumption is flawed and adversarial auditors can manipulate XAI explanations through manipulation attacks such as output shuffling or scaffolding out-of-distribution (OOD) to conceal model biases while maintaining high prediction accuracy aiming for fairwashed explanation. In this paper, we introduce a novel defense framework, ExplainGuard, that leverages a Zero-Trust architecture (ZTA) design to be incorporated within the XAI explanation supply chain and ensures the integrity of the generated explanation. This framework would help us to replace the ambiguous default assumption of "auditor is trustworthy," with a continuous "verify-then-trust" approach. Our design architecture establishes a Policy Decision Point (PDP) that enforces three distinct pillars of verification before any explanation is released to the user: (1) asset integrity via behavioral fingerprint to detect model substitution, (2) semantic validity using axiomatic consistency checks to reject mathematically impossible explanations, and (3) feature faithfulness verification utilizing a ranking stability approach with minimal computational overhead. Finally, we evaluate how ExplainGuard can effectively neutralize state- of-the-art explanation manipulation attacks while transforming the auditing process into a verifiable operation.

==> methodology.tex <==
% \subsection{Verification Authority Description (SecureXAI Framework)}

% % The Verifier ($\mathbf{V}$) acts as the immutable trust anchor by controlling the secure environment, managing cryptographic keys, and executing the non-repudiable verification protocols.

% % \subsection{Operational Protocol and Key Management}
% % \begin{enumerate}
% %     \item \textbf{Registration:} The Model Owner ($\mathbf{E}$) registers the black-box model ($f$) with the Verifier, considering model developer providing the secret watermark inputs ($I_c$) and receiving an authenticated Model Hash ($H$) and cryptographic key pair for the owner.
% %     \item \textbf{Authorization:} $\mathbf{E}$ issues a unique, request-specific API key ($K_A$) to the Auditor ($\mathbf{A}$), linked to the model $f$ and a specific Request ID $R_{id}$.
% %     \item \textbf{Submission:} $\mathbf{A}$ submits a structured data package containing the calculated SHAP values ($\Phi_A$) and the KernelSHAP explainer object ($E_{explainer}$), serialized and encrypted in a restricted, non-executable format, using $K_A$.
% % \end{enumerate}

% \subsection{Main Task 1: Verifying Model and Function Integrity}

% This task ensures that the explanation is generated by the original, authorized model ($M$) and that the specific function being audited is the one extracted from the Auditor's submitted explainer object ($E_{explainer}$).

% \subsection{Model Integrity Check: Behavioral Watermarking}
% To defeat model substitution attacks, the Verifier implements a behavioral watermarking defense \cite{[6]}.
% \begin{itemize}
%     \item $\mathbf{V}$ stores a confidential set of watermark input samples ($W$). These samples are specifically crafted to lie near decision boundaries or be slightly out-of-distribution (OOD) to maximize the behavioral divergence between the true model ($M$) and any adversarial clone ($M'$) \cite{[7, 8, 9]}.
%     \item $\mathbf{V}$ uses the trusted model $M$ to calculate the expected deterministic hash ($H_V$) based on the prediction probabilities ($P(y|W)$) for $W$ \cite{[10, 11]}.
%     \item During an audit, $\mathbf{V}$ queries the black-box API for predictions on $W$ and compares the resulting hash ($H_A$) against $H_V$. Any substantial discrepancy (exceeding a tight, predefined tolerance) triggers a Model alteration Flag, confirming the use of an unauthorized model \cite{[12]}.
% \end{itemize}



% \subsubsection{Logical Proof: Linking SHAP Values to Explainer Function}
% The Verifier must confirm that the submitted SHAP values ($\Phi_A$) correspond to the specific prediction function $f(x)$ embedded within the explainer object \cite{[13]}.

% \begin{enumerate}
%     \item \textbf{Function Extraction:} After safe deserialization (see Section 6), $\mathbf{V}$ extracts the canonical prediction function $f(x)$ from $E_{explainer}$ (e.g., `explainer.model.predict\_proba`) \cite{[13, 14]}.
%     \item \textbf{Identity Verification:} This hash is compared against the known, authorized hash ($H$) of the Model Owner's model $M$ registered with the Verifier. A match confirms that the function used in the explainer is mathematically identical to the expected, authorized function $M$ \cite{[17]}.
%     \item \textbf{Axiomatic Check (Tier 1):} The extracted function $f(x)$ is immediately used to perform the Axiomatic Consistency Check. This check definitively links the $\Phi_A$ to the explainer's function: if the axiom fails, the submitted $\Phi_A$ are not mathematically consistent with the model function extracted from $E_{explainer}$.
% \end{enumerate}
% This process ensures that if an attacker substitutes the true model with a wrapper $M'$ inside the explainer object ($E_{explainer}$), the identity verification in Step 3 fails. If the attacker generates random SHAP values ($\Phi_A$) from the correct $M$, the Axiomatic Check in Step 4 will catch the inconsistency.

% \subsection{Main Task 2: Verifying Standard SHAP Library Usage}

% To avoid performing a full recalculation that would negate the Auditor's role, $\mathbf{V}$ employs a multi-tiered, statistical sampling approach focused on high-impact features and cross-method consistency. This ensures the Auditor used a standard SHAP methodology without manipulating the results, rather than submitting random values \cite{[18, 19]}.

% \subsection{Tier 1: Low-Cost Axiomatic Consistency Check}
% This check exploits the core Local Accuracy Axiom of SHAP \cite{[20, 21, 22]}: the sum of all feature attributions ($\phi_i$) must equal the difference between the actual prediction $f(x)$ and the baseline expected value ($\phi_0$).

% $$\sum_{i=1}^{M} \phi_i = f(x) - \phi_0$$
% \begin{itemize}
%     \item $\mathbf{V}$ executes the model function $f(x)$ (extracted and verified in Task 1) on the input instance $x$ to get $f(x)_V$.
%     \item $\mathbf{V}$ calculates the difference: $\mathbf{Error} = \left| \sum \Phi_{A,i} - (f(x)_V - \phi_0) \right|$.
%     \item Since this is a check against a fundamental axiom, the tolerance ($\epsilon$) is extremely tight, based only on machine floating-point precision \cite{[23, 24]}. Any failure indicates mathematical inconsistency or trivial randomization of $\Phi_A$.
% \end{itemize}

% \subsection{Tier 2: Partial Feature Attribution Audit (Top-k TkIP)}
% To verify fidelity without full recalculation, $\mathbf{V}$ performs an efficient, targeted statistical audit on a small sample of critical instances ($X_{audit}$).

% \begin{itemize}
%     \item \textbf{Audit Set Selection:} $\mathbf{V}$ selects samples near the model's decision boundary or those with low prediction confidence, as these instances are most susceptible to explanation manipulation \cite{[20, 25]}.
%     \item \textbf{MAB-Based Partial Recalculation:} $\mathbf{V}$ does not perform full KernelSHAP, but rather employs the Top-k Identification Problem (TkIP) approach, which leverages Multi-Armed Bandit (MAB) algorithms \cite{[26, 27]}. This approach drastically reduces the required number of model queries (up to $40\times$ efficiency gain) by focusing sampling resources only on the $k$ most important features whose ranking needs verification \cite{[26, 18, 28]}.
%     \item \textbf{Fidelity Comparison:} $\mathbf{V}$ compares the Auditor's submitted Top-k SHAP values ($\Phi_A$) against the partially recalculated values ($\Phi_V$) using:
%     \begin{itemize}
%         \item \textbf{Rank Correlation ($\rho$):} Ensures the relative feature ordering is preserved. A low $\rho$ indicates structural manipulation \cite{[29, 30]}.
%         \item \textbf{Top-k Identification Accuracy:} Verifies that the most critical features identified by $\mathbf{A}$ match the verified set $\Phi_V$ \cite{[31, 32]}.
%     \end{itemize}
% \end{itemize}
% This partial approach satisfies the need for verification while involving the Auditor in the overall explanation generation process.




